Impact of Social Learning on Privacy-Preserving Data Collection

We study a model where a data collector obtains data from users through a payment mechanism, aiming to learn the underlying state from the elicited data. The private signal of each user represents her knowledge about the state; and through social interactions each user can also learn noisy versions of her social friends' signals, which is called `learned group signals'. Thanks to social learning, users have richer information about the state beyond their private signals. Based on both her private signal and learned group signals, each user makes strategic decisions to report a privacy-preserved version of her data to the data collector. We develop a Bayesian game theoretic framework to study the impact of social learning on users' data reporting strategies and devise the payment mechanism for the data collector accordingly. Our findings reveal that, in general, the desired data reporting strategy at the Bayesian-Nash equilibrium can be in the form of either a symmetric randomized response (SR) strategy or an informative non-disclosive (ND) strategy. Specifically, a generalized majority voting rule is applied by each user to her noisy group signals to determine which strategy to follow. Further, when a user plays the ND strategy, she reports privacy-preserving data completely based on her group signals, independent of her private signal, which indicates that her privacy cost is zero. We emphasize that the reported data when a user plays the ND strategy is still informative about the underlying state because it is based on her learned group signals. As a result, both the data collector and the users can benefit from social learning which drives down the privacy costs and helps to improve the state estimation at a given payment budget. We further derive bounds on the minimum total payment required to achieve a given level of state estimation accuracy.

==> selfCentered.tex <==
\section{Bayesian Nash Equilibrium: The Case with Self-Interested Users}

In this setting, we consider the case where the users do not provide any privacy guarantees to their peers and their sole privacy concern is restricted to their own private signals $S_i$'s. This setting presents an obstacle and an opportunity for the data collector. When this setting is compared to the market model in the absence of social ties \cite{Wang2016Report}, the privacy-aware individuals have additional information to devise their strategies and can possibly increase their expected rewards. On the other hand, the individuals' report can become more informative albeit it might imply they leak their friends' signals since they are not concerned about their friends' privacy.

For a user $i$, imagine an extreme situation where nearly all of the bits she receive through her social ties are bit 1. If she has sufficiently many friends, she can confidently predict that the underlying state $W$ is very likely to be 1 purely based on her group signal $C_i$ and without including her own signal $S_i$: $\hat{W}_i(C_i) \teq 1$. She can further argue that, based on her group signal observation, it is more likely that the majority of the users also predict the underlying state to be 1 (since the quality parameters $\theta_0,\theta_1 > 0.5$). This strategy sets her privacy cost to 0 since her prediction $\hat{W}_i$ is independent from her private signal $S_i$. On the other hand, imagine another extreme case where the number of 1s and 0s in the $C_i$ are almost equal. In this case, the user could improve her expected utility by including $S_i$ in her prediction, i.e. $S_i$ could be the "tie-breaking vote". The former strategy is later referred as \textit{non-disclosive} and the latter is called as \textit{randomized symmetric}. 

In general, the set of mixed strategies $\triangle(\mathcal{X})$ is uncountable. Lemma~\ref{symconcinflemma} characterize the Nash equilibrium strategies and reduces the set of possible equilibriums. We first formalize the definitions of symmetric randomization and non-disclosive strategies.
\begin{definition}
$\sigma_i([S_i \ C_i])$ is called a non-disclosive strategy, if it satisfies the following where $c_i \in \{0,1\}^{d}$ and $s_i, x_i \in \{0,1 \}$:
\begin{align*}
& \Pr_{\sigma_i} (X_i = x_i | S_i = 1, C_i = c_i) = \Pr_{\sigma_i} (X_i = x_i | S_i = 0, C_i = c_i), \\
& \Pr_{\sigma_i} (X_i = \bot | S_i = s_i, C_i = c_i) = 0.
\end{align*}
\end{definition}
When a non-disclosive strategy is played by user $i$, the report $X_i$ is independent from the private signal $S_i$. This sets her privacy cost to 0 since she is self-interested and privacy-aware of only her own signal. Notice that her report can still depend on her group signal $C_i$ and be correlated with the underlying state $W$. If a user plays with a strategy where her report $X_i$ is independent from both her private data $S_i$ and her group signal $C_i$, then $X_i$ is pure noise for the data collector and it can degrade the estimation performance of the underlying state $W$. We call such strategies as \textit{non-informative} \cite{Wang16}. In the absence of the social ties ($D_i = 0$), non-disclosive strategies certainly yield pure noise reported data. 
\begin{definition}
$\sigma_i([S_i \ C_i])$ is called a symmetric randomization strategy, if it satisfies the following where $c_i \in \{0,1\}^{d}, D_i \teq d$:
\begin{align*}
& \Pr_{\sigma_i} (X_i = 1 | S_i = 1, C_i = c_i)  = \Pr_{\sigma_i} (X_i = 0 | S_i = 0, C_i = c_i), \\
 & \Pr_{\sigma_i} (X_i = \bot | S_i = 1, C_i = c_i) = \Pr_{\sigma_i} (X_i = \bot | S_i = 0, C_i = c_i) = 0.
\end{align*}
\end{definition}
When a user does not possess social ties ($D_i = 0$), playing with a symmetric randomized strategy corresponds to the privacy-preserved truthful reporting her own signal $S_i$ where she can control the privacy level, or from a different perspective the injected noise level. In the existence of social ties, this strategy can still be adopted when that particular group signal realization $c_i$ is not "informative" for the user. 
\begin{lemma}
\label{symconcinflemma}
Consider a payment mechanism in which the payment is zero for non-participating individuals ($X_i = \bot$) and positive for participating individuals $(X_i \in \{ 0,1\})$. Then, $\sigma_i(\cdot)$ in a Bayesian equilibrium is a symmetric randomization strategy or a non-disclosive strategy.
\end{lemma}

\subsection{Analysis of Majority Voting Payment Mechanisms}

Building an explicit, non-negative payment system to incentivize truthful strategies is a challenge. The objective outcome, namely $W$ is neither available to the data collector nor to the users. The idea that the data collector can utilize the correlation in users' private information to bring about truthful strategies is analyzed in detail in the literature as peer-prediction methods  \cite{Miller04} (see \cite{FaltingsBook17} for an extensive survey of this field). In other words, the data collector can use the reports from all the other users ($-i$) to evaluate user $i$'s report and determine her reward respectively. In the framework of the data privacy games, however, the users have privacy concerns. A variant of the peer-prediction method is employed in \cite{Wang2016Report} where the possibility of having social ties among the users are not considered. In this proposed framework, the users observe more erroneous samples of $W$, their friends' signals, in addition to their own private information. Hence, the users have more information to determine their decision strategies and this constitutes an additional challenge for the data collector. Remember that the degree distribution $\rho(k)$ is the only public information data collector knows about the social graph. Note that the investigation of possible countermeasures which can be taken by the data collector in this new framework is still an open problem. With these remarks, a modified version of the majority payment mechanism from \cite{Wang2016Report} is proposed as $\tilde{\mathbf{R}}(\mathbf{X})$:

\begin{enumerate}
\item Each user reports her data and the data collector counts the number of participants $n$ excluding the users with "non-participation" data reports.
\item For non-participating users, the payment is zero. If $n = 1$, pay zero to this participant. Otherwise, for each participating user $i$, compute the majority of the other participants' reported data.
\begin{equation*}
M_{-i} =
\left\{ \begin{array}{ll}
         1 & \text{ if } \sum \limits_{j: x_j \neq \bot, j \neq i} x_j > \left \lfloor{\frac{n}{2}}\right \rfloor ;\\
        0 & \mbox{ otherwise}.\end{array} \right.
\end{equation*}
\item Compute the payment user $i$ receives:
\begin{align}
\tilde{R}_i & (1,\mathbf{x}_{-i}) = Z \big ( p_W(1) (1- \beta) + p_W(0) \beta \big ) M_{-i}, \label{PaymentMech1} \\
\tilde{R}_i & (0,\mathbf{x}_{-i}) = Z \big ( p_W(0) (1- \beta) + p_W(1) \beta \big )  (1-M_{-i}) \label{PaymentMech2}
\end{align}
\end{enumerate}
It is easy to verify that the proposed majority payment mechanism $\tilde{\mathbf{R}}(\mathbf{X})$ is nonnegative if $Z>0$ and $\beta > 0.5$. Denote $F_i = \sum_{j \in G_i} C_{ij}$ (sum of the components of the group signal vector $C_i$) \footnote{ Note that $F_i$ is the sufficient statistics for the prediction of the underlying state $W$ by the individual $i$.}. To simplify notation, for a given user strategy $\sigma_i^*$ define $p_{s_i,f_i}$ and $q_{s_i,f_i}$ as the following:
\begin{align*}
p_{s_i,f_i} & = \Pr_{\sigma_i^*} (X_i \teq 1 | S_i \teq 1, F_i \teq f_i) \\
q_{s_i,f_i} & = \Pr_{\sigma_i^*} (X_i \teq 0 | S_i \teq 1, F_i \teq f_i)
\end{align*}
\subsection{Noiseless Group Signals}
In this subsection, we analyze the case where the users receive noiseless versions of their friends' signals where the crossover probability $\alpha \teq 0$. The quality of their own signal $S_i$ and received signals $C_{ij}$'s are equal: $\theta_1 \teq \theta_0$. The Theorem~\ref{NEThm1} specifies a Bayesian equilibrium where users decide between following a majority voting strategy \eqref{NoiselessMV} or a symmetric randomization strategy \eqref{NoiselessSR}. The users seek a $\textit{simple majority}$ within their social signal $C_i$ and report that majority signal. If the number of $1s$ is greater than the number of $0s$ in $C_i$, then their report $X_i \teq 1$ with probability 1, and vice versa.
\begin{theorem}
\label{NEThm1}
In the large $N$ where every user is self-interested, for a specified degree distribution $\rho(k)$ with $E(D_j^2) << N$  $\forall j \in \mathcal{I}$, for the payment mechanism defined in \eqref{PaymentMech1} and \eqref{PaymentMech2}, for crossover probability $\alpha \teq 0$, if the data collector chooses $\beta = P_{\mathbf{\sigma}^*} (M_{i} \! = \! 1 | W \!= \!1)$, and  $Z = g'(\epsilon)(e^\epsilon+1)^2/[2e^\epsilon(1-2\beta)(1-2\theta)p_W(1)p_W(0)]$ then there exists a Bayesian Nash equilibrium $\mathbf{\sigma}*$ where $D_i = d$:
\begin{subequations}
\label{NoiselessMV}
\begin{align}
& \text{If } f_i > d/2; \ p_{1,f_i} = p_{0,f_i} = 1, \ q_{1,f_i} = q_{0,f_i} = 0. \\
& \text{If } f_i < d/2; \ p_{1,f_i} = p_{0,f_i} = 0, \ q_{1,f_i} = q_{0,f_i} = 1,
\end{align}
\end{subequations}
\begin{equation}
\label{NoiselessSR}
\text{Else }; \ p_{1,f_i} = p_{0,f_i} = e^{\epsilon}/(1+e^{\epsilon}), \ q_{1,f_i} = q_{0,f_i} = 1/(1+e^{\epsilon}).
\end{equation}
\end{theorem}
\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{Regimes.pdf}
	\caption[Two Symmetric Randomization Regimes]{Optimal report strategy vs crossover probability. Noiseless case: If $F_i = D_i/2$, the optimal strategy is symmetric randomized; otherwise, it is non-disclosive. Noisy case: If $F_i \in (D_i/2\teg A/2,D_i/2\tsum A/2)$, the optimal strategy is symmetric randomized; otherwise, it is non-disclosive.}
\end{figure}
In the case where the users are self-interested  and the crossover probability $\alpha \teq 0$, consider a scenario where $i$ has $2k \tsum 1$ friends and $j$ is one of them. Define $F_{i,-j} \teq \sum_{\ell \in G_i-\{j\}}$. At the Bayesian equilibrium defined in the Theorem~\ref{NEThm1}, given $F_{i,-j} = k$, user $j$'s private signal is completely disclosed by the reporting strategy of her friend $i$: $\Pr_{\sigma_i^*} (X_i \teq 1 | S_i \teq s_i,F_{i,-j} \teq k, S_{ij} \teq 1) \teq 1$ and $\Pr_{\sigma_i^*} (X_i \teq 0 | S_i \teq s_i,F_{i,-j} \teq k, S_{ij} \teq 0) \teq 1$.

\subsection{Noisy Group Signals}
In this subsection, we analyze the case where the users receive noisy versions of their friends' signals. This creates a discrepancy between the quality of their own signal $S_i$ and received signals $C_{ij}$'s: $\theta_1 < \theta_0$. Theorem \ref{UCEqForm} specifies a Bayesian equilibrium where users decide between following the majority voting strategy \eqref{NoisyMV} or a symmetric randomization strategy \eqref{NoisySR} depending on the \textit{strength} of information they receive through their social links. Users seek a \textit{super majority}, a specified level of support which is greater than the threshold of one half which is sought in simple majority, within their social signal $C_i$. In the absence of a super majority, the users follow symmetric randomization strategies \eqref{NoisySR} where the privacy level $\xi(\cdot)$ can depend on the number of $1s$ (or equivalently $0s$) in $C_i$. In other words, when $\alpha > 0$, there exists a symmetric randomization interval within possible values of $F_i$, which is the sum of $1$s in the group signal. 

\begin{theorem}
\label{UCEqForm}
For the user-centric case, for a sparse social graph with large $N$, for the payment mechanism defined in \eqref{PaymentMech1} and \eqref{PaymentMech2} if the data collector chooses $\beta = P_{\mathbf{\sigma}^*} (M_{i} \! = \! 1 | W \!= \!1)$, and  $Z = 2 g'(\epsilon)(e^\epsilon+1)^2/[e^\epsilon(1-2\beta)(1-2\theta)]$ then there exists a  Bayesian Nash equilibrium strategy profile $\mathbf{\sigma}^*(\cdot)$ in the following form:
\begin{subequations}
\label{NoisyMV}
\begin{align}
\text{If } & f_i > (d_i\tsum \tau_1)/2; \ p_{1,f_i} = p_{0,f_i} = 1, \ q_{1,f_i} = q_{0,f_i} = 0. \\
\text{If } & f_i < (d_i\teg \tau_0)/2; \ p_{1,f_i} = p_{0,f_i} = 0, \ q_{1,f_i} = q_{0,f_i} = 1,
\end{align}
\end{subequations}
\begin{equation}
\label{NoisySR}
\text{Else;} \ p_{1,f_i} \teq p_{0,f_i} \teq \frac{e^{\xi(f_i)}}{1+e^{\xi(f_i)}}, \ q_{1,f_i} \teq q_{0,f_i} \teq \frac{1}{1+e^{\xi(f_i)}}.
\end{equation}
where $d_i$ is given as the number of friends user $i$ has; $0 \leq \tau_0,\tau_1 \leq d_i$; $f_i \in \{0,1,\dots,d_i\}$ and $\xi(f_i) \geq 0$; $p_{s_i,f_i}\teq \Pr_{\sigma_i^*} (X_i \teq 1 | S_i \teq s_i, F_i \teq f_i)$ and $q_{s_i,f_i} \teq \Pr_{\sigma_i^*} (X_i \teq 0 | S_i \teq s_i, F_i \teq f_i)$. 
\end{theorem}

If there are equal priors, i.e., $p_W(1) \teq p_W(1) \teq 0.5$, the analytic expressions for $\tau_0$, $\tau_1$ and $\xi(f_i)$ can be simplified. In this special case, we find privacy level to be independent from $f_i$ and equal to $\epsilon$ parameter of the payment mechanism. As an interesting observation, it should be noted that, in this special case, the impact of the social signal on the equilibrium strategy is none when $f_i$ is in the symmetric randomization region.

\begin{corollary}
For the equilibrium strategy form expressed in Theorem \ref{UCEqForm}, if there is equal priors $p_W(0) \teq p_W(1) \teq 0.5$, then $\xi(f_i) \teq \epsilon$ and $\tau_0 \teq \tau_1 \teq \tau$ where
\begin{equation*}
\tau \teq \log \Bigg ( \frac{e^\epsilon[e^\epsilon \theta_0 \tsum 1 \teg (2\theta_0 \teg 1)g(\epsilon)/g'(\epsilon)]\tsum 1\teg \theta_0}{e^\epsilon[e^\epsilon (1\teg \theta_0) \tsum 1 \tsum (2\theta_0\teg 1)g(\epsilon)/g'(\epsilon)]\tsum \theta_0} \Bigg ) \Bigg / \log \Bigg ( \frac{\theta_1}{1-\theta_1} \Bigg ).
\end{equation*}
\end{corollary}

When there are no equal priors, it is not possible to precisely express the privacy level function $\xi(f_i)$ and the threshold parameters $\tau_0$ and $\tau_1$, as functions of system parameters $\alpha$, $p_W(0)$, $g(\cdot)$ and $\theta_0$. However, their computation is not challenging.

\begin{equation}
B_0 = \frac{\log(\theta_0/(1-\theta_0))}{\log(\theta_1/(1-\theta_1))}, \ B_1 = \frac{\log(\theta_0/(1-\theta_0))}{\log(\theta_1/(1-\theta_1))}
\end{equation}

\begin{equation}
h(\xi) \teq g'(\epsilon)e^{\xi \hspace{-0.2mm} \teg \epsilon} \hspace{-1mm} \left(\frac{e^\epsilon\tsum 1}{e^{\xi}\tsum 1}\right)^2 \hspace{-2mm} \frac{(1\tsum (\theta_1/(1\teg\theta_1))^{d\teg 2f})/2}{1 \tsum p_W(0)((\theta_1/(1\teg\theta_1))^{d\teg 2f}\teg \hspace{-0.2mm}1)} \hspace{0.2mm} \teg g'(\xi) \hspace{-0.5mm} \label{optSREquation}
\end{equation}

\begin{equation*}
Y_\ell = \frac{\log (\tau_\ell)}{\log (\theta_1/(1 \teg \theta_1))}, \ell \teq 0,1 \text{ and } Z =  (2\theta_0 \teg 1) 2e^\epsilon \frac{g(\xi^*)}{g'(\epsilon)} \frac{(e^{\xi^*}\tsum 1)}{(e^\epsilon \tsum 1)^2}, 
\end{equation*}

\begin{equation}
A_0(\xi) \teq \frac{e^{\xi} \theta_0 \tsum 1 \teg \theta_0 \teg p_W(1) Z}{e^{\xi} (1\teg \theta_0) \tsum \theta_0 \tsum p_W(0) Z},
A_1(\xi) \teq \frac{e^{\xi} (1\teg \theta_0) \tsum \theta_0 \tsum p_W(1) Z}{e^{\xi} \theta_0 \tsum 1 \teg \theta_0 \teg p_W(0) Z}
\end{equation}

\begin{algorithmic}
\FOR{$f=0$ to $d$} 
	\IF{$0 \leq f \leq ( d \teg B_0 )/2$}
 		\STATE Play majority voting
 	\ELSIF{$( d \teg B_0)/2 < f < d/2$}
 		\STATE Solve for $h(\xi^*) \teq 0$ from \eqref{optSREquation} and set $\xi(f_i) \teq \xi^*$
        \IF{$A_0(\xi^*) > 0$}
        	\STATE Play Symmetric Randomized with $\xi^*$
            	\ELSE
                \STATE Play Majority Voting
                \ENDIF
\ELSIF{$ d/2 < f < ( d \tsum B_0)/2$}
 		\STATE Solve for $h(\xi^*) \teq 0$ from \eqref{optSREquation} and set $\xi(f_i) \teq \xi^*$
        \IF{$A_1(\xi^*) > 0$}
        	\STATE Play Symmetric Randomized with $\xi^*$
            	\ELSE
                \STATE Play Majority Voting
                \ENDIF
        \ELSE
        \STATE Play Majority Voting
 \ENDIF
\ENDFOR
\end{algorithmic}

% \begin{theorem}
% \label{NEThm2}
% In the large $N$ where every user is self-interested, for a specified degree distribution $\rho(k)$ with $E(D_j^2) << N$  $\forall j \in \mathcal{I}$, for the payment mechanism defined in \eqref{PaymentMech1} and \eqref{PaymentMech2}, and $p_W(0) \teq p_W(1) \teq 0.5 $ if the data collector chooses $\beta = P_{\mathbf{\sigma}^*} (M_{i} \! = \! 1 | W \!= \!1)$, and  $Z = 2 g'(\epsilon)(e^\epsilon+1)^2/[e^\epsilon(1-2\beta)(1-2\theta)]$ then there exists a Bayesian Nash equilibrium $\mathbf{\sigma}*$ where $D_i = d$:
% \begin{align*}
% & \text{If } f_i > (d+A)/2; \ p_{1,f_i} = p_{0,f_i} = 1, \ q_{1,f_i} = q_{0,f_i} = 0. \\
% & \text{If } f_i < (d-A)/2; \ p_{1,f_i} = p_{0,f_i} = 0, \ q_{1,f_i} = q_{0,f_i} = 1. \\
% & \text{Else };\ p_{1,f_i} = p_{0,f_i} = e^{\epsilon}/(1+e^{\epsilon}), \ q_{1,f_i} = q_{0,f_i} = 1/(1+e^{\epsilon}).
% \end{align*}
% where
% \begin{equation*}
% A \teq \log \Bigg ( \frac{e^\epsilon[e^\epsilon \theta_0 \tsum 1 \teg (2\theta_0 \teg 1)g(\epsilon)/g'(\epsilon)]\tsum 1\teg \theta_0}{e^\epsilon[e^\epsilon (1\teg \theta_0) \tsum 1 \tsum (2\theta_0\teg 1)g(\epsilon)/g'(\epsilon)]\tsum \theta_0} \Bigg ) \Bigg / \log \Bigg ( \frac{\theta_1}{1-\theta_1} \Bigg ).
% \end{equation*}
% \end{theorem}

% The equal priors condition can be relaxed:
% \begin{proposition}
% In the large $N$, for the user-centric case, for a specified degree distribution $\rho(k)$ with $E(D_j^2) << N$  $\forall j \in \mathcal{I}$, for the payment mechanism defined in \eqref{PaymentMech1} and \eqref{PaymentMech2} if the data collector chooses $\beta = P_{\mathbf{\sigma}^*} (M_{i} \! = \! 1 | W \!= \!1)$, and  $Z = 2 g'(\epsilon)(e^\epsilon+1)^2/[e^\epsilon(1-2\beta)(1-2\theta)]$ then there exists a Bayesian Nash equilibrium $\mathbf{\sigma}*$ where $D_i = d$:
% \begin{align*}
% & \text{If } f_i > (d+A_1)/2; \ p_{1,f_i} = p_{0,f_i} = 1, \ q_{1,f_i} = q_{0,f_i} = 0. \\
% & \text{If } f_i < (d-A_0)/2; \ p_{1,f_i} = p_{0,f_i} = 0, \ q_{1,f_i} = q_{0,f_i} = 1, \\
% & \text{Else };\ p_{1,f_i} = p_{0,f_i} = e^{\xi^*}/(1+e^{\xi^*}), \ q_{1,f_i} = q_{0,f_i} = 1/(1+e^{\xi^*}).
% \end{align*}
% where 
% \begin{equation*}
% A_\ell = \frac{\log (\tau_\ell)}{\log (\theta_1/(1 \teg \theta_1))}, \ell \teq 0,1 \text{ and } B =  (2\theta_0 \teg 1) 2e^\epsilon \frac{g(\xi^*)}{g'(\epsilon)} \frac{(e^{\xi^*}\tsum 1)}{(e^\epsilon \tsum 1)^2}, 
% \end{equation*}
% \begin{equation*}
% \tau_0 = \frac{e^{\xi^*} \theta_0 \tsum 1 \teg \theta_0 \teg p_W(1) B}{e^{\xi^*} (1\teg \theta_0) \tsum \theta_0 \tsum p_W(0) B},
% \tau_1 = \frac{e^{\xi^*} (1\teg \theta_0) \tsum \theta_0 \tsum p_W(1) B}{e^{\xi^*} \theta_0 \tsum 1 \teg \theta_0 \teg p_W(0) B}.
% \end{equation*}

% To compute $\xi^*$, solve the Equation \eqref{optSREquation} for each $f$:
% \begin{equation}
% g'(\epsilon)e^{\xi^* \hspace{-0.5mm} \teg \epsilon} \hspace{-1mm} \left(\frac{e^\epsilon\tsum 1}{e^{\xi^*}\tsum 1}\right)^2 \hspace{-2mm} \frac{(1\tsum (\theta_1/(1\teg\theta_1))^{d\teg 2f})/2}{1 \tsum p_W(0)((\theta_1/(1\teg\theta_1))^{d\teg 2f}\teg 1)} \hspace{0.5mm} \teg g'(\xi^*) \teq 0. \label{optSREquation}
% \end{equation}
% \end{proposition}

\textit{Remark:} To derive an explicit expression for $\xi^*$, apply first order Taylor expansions at point $\epsilon$ on $g'(\xi^*) \cong g'(\epsilon) \tsum (\xi^*\teg \epsilon) g''(\epsilon)$ and $ e^{\xi^* \teg \epsilon} (e^\epsilon\tsum 1 / (e^{\xi^*}+1))^2 \cong 1\teg (\xi^*\teg \epsilon) ((e^\epsilon\teg 1)/(e^\epsilon\tsum 1))$ and solve the equation \eqref{optSREquation}:
\begin{equation}
\xi^* = \epsilon + (2p_W(0)\teg 1) \frac{\frac{(1\teg (\theta_1/(1\teg\theta_1))^{d\teg 2f})/2}{1 \tsum p_W(0)((\theta_1/(1\teg\theta_1))^{d\teg 2f}\teg 1)}}{\frac{(1\tsum (\theta_1/(1\teg\theta_1))^{d\teg 2f})/2}{1 \tsum p_W(0)((\theta_1/(1\teg\theta_1))^{d\teg 2f}\teg 1)}\frac{e^\epsilon\teg 1}{e^\epsilon\tsum 1}\tsum \frac{g''(\epsilon)}{g'(\epsilon)}}. \label{linSR}
\end{equation}

In the Equation \eqref{linSR}, we can observe that three important parameters impact the shift of $\xi^*$ from $\epsilon$: $\epsilon, p_W(0)$ and $g''(\epsilon)$. For equal priors, the deviation from $\epsilon$ is zero and $\xi^* \teq \epsilon$. The linear approximation also satisfies this and the deviation from $\epsilon$ becomes negligible as $p_W(0)$ approaches to 0.5.  $\xi^*$ could be approximated with $\epsilon$ as the cost function $g''(\epsilon)$ becomes more and more convex, i.e. $g''(\epsilon)/g'(\epsilon)$ increases. As $\epsilon$ increases, $(e^\epsilon\teg 1)/(e^\epsilon\tsum 1)$ goes to 1. 

In the case where the users are still self-interested but the crossover probability $\alpha > 0$, the privacy leakage through social links is more restricted but it could still be critical. Consider a scenario where $i$ has $d$ friends and $j$ is one of them. At the Bayesian equilibrium defined in the Theorem~\ref{NEThm2}, given $F_{i,-j} \teq k$ and $1\tsum(d\teg A)/2 \leq k < (d\teg A)/2$, the disclosiveness of user $j$'s private signal  by the reporting strategy of her friend $i$ can be quantified as: $\Pr_{\sigma_i^*} (X_i \teq 1 | S_i \teq 1, F_{i,-j} \teq k, S_{ij} \teq 1) \teq \alpha e^{\epsilon}/(1+e^{\epsilon})$ and $\Pr_{\sigma_i^*} (X_i \teq 0 | S_i \teq 1, F_{i,-j} \teq k, S_{ij} \teq 0) \teq \alpha \tsum (1\teg \alpha)e^{\epsilon}/(1+e^{\epsilon})$. It improves the privacy leakage of user $j$ very significantly when we compare it with $\alpha \teq 0$ case.
